Hydrogen in Disordered Titania: Connecting Local Chemistry, Structure, and Stoichiometry through Accelerated Exploration

Hydrogen incorporation in native surface oxides of metal alloys often controls the onset of metal hydriding, with implications for materials corrosion and hydrogen storage. A key representative example is titania, which forms as a passivating layer on a variety of titanium alloys for structural and functional applications. These oxides tend to be structurally diverse, featuring polymorphic phases, grain boundaries, and amorphous regions that generate a disparate set of unique local environments for hydrogen. Here, we introduce a workflow that can efficiently and accurately navigate this complexity. First, a machine learning force field, trained on ab initio molecular dynamics simulations, was used to generate amorphous configurations. Density functional theory calculations were then performed on these structures to identify local oxygen environments, which were compared against experimental observations. Second, to classify subtle differences across the disordered configuration space, we employ a graph-based sampling procedure. Finally, local hydrogen binding energies are computed using exhaustive density functional theory calculations on representative configurations. We leverage this methodology to show that hydrogen binding energetics are described by local oxygen coordination, which in turn is affected by stoichiometry. Together these results imply that hydrogen incorporation and transport in TiO$_x$ can be tailored through compositional engineering, with implications for improving performance and durability of titanium-derived alloys in hydrogen environments.

==> Sections/results.tex <==
\section{Results}

\subsection{Generation and validation of amorphous TiO$_2$ structures}

\begin{figure}
       \centering
    	\includegraphics[trim={0 0cm 0 0cm},width=1.0\textwidth]{Figures/all_struct_validation.pdf}
    	\caption{(a) Experimental NMR spectra calculated using a prepared amorphous titania sample. (b) Distribution of computed isotropic chemical shift ($\delta_{iso}$) for O in a-TiO$_{2}$. Colors define $\delta_{iso}$ for different oxygen coordination numbers, as defined by the corresponding labels in (b). The dashed vertical line represents the $\delta_{iso}$ for a 3F oxygen atom in crystalline anatase TiO$_{2}$.  (c) Molecular dynamics derived time-averaged pair-correlation function of amorphous TiO$_{2}$ at T=2250K, for both DFT and the AFNN. The pair-correlation function is decomposed based on chemical species interactions (colors, with identifying labels). The AFNN is shown as the solid line, while DFT is given as a dashed line. (d) The vibrational density of states, derived from molecular dynamics simulations at T=2250K, for DFT (light blue) and the AFNN (pink). In both scenarios, DFT calculations were performed on 216 atoms, while AFNN simulations were performed using 1944 atoms.}
    \label{fig:structure_val}
\end{figure}

As a first step, it is critical to introduce a benchmark against which our model of disordered TiO$_{2}$ can be validated. Accordingly, we produced a representative sample of amorphous TiO$_{2}$ powders using a sol-gel method (see Experimental Methods for details). The sample was characterized using $^{17}$O solid-state NMR, which provides a spectroscopic ``fingerprint'' that can also be directly computed from our computational representation (additional XPS measurements can be found in the Supporting Information). Figure~\ref{fig:structure_val}(a) shows the experimentally measured $^{17}$O NMR isotropic chemical shifts on the amorphous powder, in which three distinct peaks at 718 ppm, 545 ppm, and 383 ppm can be identified. This implies that three distinct oxygen environments exist within the disordered TiO$_2$ material, each of which should be reproduced in a properly generated model. 

Next, we proceeded to generate a range of configurations that capture these same local environments in atomistic TiO$_2$ models. Because the range and complexity of the amorphous configurations requires an efficient method for computing atomic forces, we developed an AFNN to rapidly generate structures. A 1944-atom system was used to validate the AFNN against 216-atom DFT simulations (a comparison between DFT and AFNN results for identically sized 96-atom systems can be found in the Supporting Information). Figure  \ref{fig:structure_val} (c) shows AFNN and DFT predictions of the time-averaged RDF (decomposed into $i-j$ species interactions), calculated from MD simulations, and (d) vibrational density of states. Overall, the AFNN RDF is in good agreement with the DFT RDF, other than slight variations in the interatomic distances. It should be noted that the AFNN simulations cover a much larger region of the TiO$_{2}$ phase space than the DFT trajectories, which only contain a few hundred structures along a single trajectory. This, combined with the small difference in density, can explain the subtle shifts observed in the RDF.

%despite a slight rightward shift in the first peak of the RDF, corresponding to Ti-O interactions. This shift is connected to a small shift to the left of the O-O peak, indicating that oxygen atoms are slightly closer together in the AFNN systems. However, i

The AFNN also shows good agreement with DFT in regard to the vibrational density of states over all calculated wavenumbers. Some disagreement does exist at small wavenumbers, with the larger density predicted by the AFNN indicating a slightly more diffuse system. This is corroborated by observing the diffusion constants of both Ti and O, predicted via the mean square displacement, which show errors of a factor of 1.5 and 1.8 for Ti and O respectively, when compared to DFT. These discrepancies, however, are minimal, and indicate that the AFNN can reliably predict the vibrational behavior TiO$_{2}$ at 2250K over a wide spectrum of atomic perturbations. It is also worth noting that errors in the predicted diffusion constant values can be quite high due to the limited simulation length of DFT, and agreement within a factor of two is more than acceptable.

A similar trend exists between the AFNN and DFT with respect to the local structure predicted for cases with lower oxygen concentrations (up to TiO$_{1.88}$), indicating that one can use the AFNN to reasonably predict the correct underlying atomic environments for a range of oxygen concentrations. Detailed calculations of the mean-square displacement calculated diffusion constants for both Ti and O can be found in the supplemental information, along with a comparison between DFT and the AFNN for the non-stoichiometric case of TiO$_{1.88}$. 

Having validated the ability of the AFNN to reproduce DFT results, we generated roughly 400 different amorphous models (using the 96-atom amorphous structures generated via the AFNN's MD simulations), which gives a total of approximately 30,000 $\delta_{iso}$ local environments for O sites. The O isotropic chemical shifts ($\delta_{iso}$) for each oxygen site was computed, as shown in Fig. \ref{fig:structure_val} (b). The results reproduce the same three-peak structure that was identified through experimental measurements. Unlike the experimental observations, our DFT NMR structure can be mapped back onto the oxygen coordination number as we have explicit atomistic structure as reference. Figure \ref{fig:structure_val}(b) shows the strong correlation between $\delta_{iso}$ for the O sites and their corresponding coordination environment. The distribution of $\delta_{iso}$ shows that it is strongly dependent on the O coordination number with the increasing $\delta_{iso}$ for the lower O coordination numbers.  

This coordination-environment dependence exists because as one decreases the number of electron-donating Ti atoms (lowering the coordination number), the electron density at the O nucleus is reduced, which deshields the nucleus and results in a larger $\delta_{iso}$.  Note that the $\delta_{iso}$ of 557 ppm for a 3F O in bulk anatase \cite{doi:10.1021/ja00021a068} is within the range of chemical shift for the 3F O in our a-TiO$_{2}$ (500-700 ppm).  The coordination dependent $\delta_{iso}$ for O was also observed from the solution $^{17}$O NMR study of titanium polyoxoalkoxide complexes, which contain 2F (OTi$_{2}$), 3F (OTi$_{3}$), and 4F (OTi$_{4}$) groups and each of which distinctly gives $\delta_{iso}$ of 650-850 ppm, 450-650 ppm, and 250-450 ppm, respectively \cite{doi:10.1021/ja00021a068}.


The ranges in chemical shift for each major peak in Fig. \ref{fig:structure_val} (a) and (b) suggest the presence of various O coordination environments in amorphous TiO$_{2}$, even within a specific CN (ex: many differnt types of 2F environments).  Based on the calculated $\delta_{iso}$ in Fig. \ref{fig:structure_val} (a), the experimental peaks at 718 ppm, 545 ppm and 383 ppm in Fig. \ref{fig:structure_val} (b) are assigned to 2F, 3F, and 4F O sites, respectively.  Note that for the 2F O coordination, the calculated $\delta_{iso}$ at 720 ppm corresponds well with the observed one, whereas there is slight overestimation of the calculated $\delta_{iso}$ for the 3F O sites at 585 ppm and 4F O sites at 460 ppm, respectively. Such minor discrepancies are common and can in principle be resolved by including an additional empirical scaling factor \cite{C4SC00083H}, but the current approach is sufficient for proper interpretation of the peak assignments. Overall, we confirm that the local coordination environment around O in our constructed amorphous TiO$_{2}$ models is highly comparable to that in the experimentally synthesized TiO$_{2}$. Quantification of the experimental peak areas reveals fractions of 14.78\%, 39.15\%, and 14.68\%. for 2F, 3F, and 4F O respectively.


%\subsection{Neural network force field validation}


\subsection{Exploration of the amorphous phase space}

Here we use the 1,944 atom amorphous trajectories, generated by the AFNN, to analyze the local atomic geometries present across the vast phase space. We use the 1,944 atom systems to perform this analysis due to the increased number of local atomic sites present when compared to the 96 atom configurations. As described earlier when validating the AFNN, the 1,944 atom trajectories provide an excellent substitute when compared to DFT, and we do not expect the local atomic environments in 1,944 atom systems to deviate significantly from those present within the 96 atom structures.

Using the AFNN-generated 1,944 atom MD trajectories, the TiO$_{x}$ phase space was characterized using the PCA decomposition of the VGOP features described earlier. Fig. \ref{fig:PCAspace}(a) shows where various values of $x$, in TiO$_{x}$, lie within this configuration space. The VGOP shows a clear separation between each case considered in this work, with some overlap existing at the outskirts of each sub-space. The TiO$_{2}$ sub-space shares some overlap with the TiO$_{1.95}$ sub-space, but does not share any portion of the total space with another value of $x$. This makes sense intuitively, as one would expect the structures encountered during a dynamic trajectory to oscillate about some equilibrium point. As the underlying structure of TiO$_{2}$ and TiO$_{1.95}$ are similar, one would expect their oscillations to overlap at the fringes of their respective sub-spaces.

\begin{figure}
       \centering
    	\includegraphics[trim={0 5cm 0 0cm},width=1.0\textwidth]{Figures/amorphous_phase_space.pdf}
    	\caption{(a) PCA-decomposed TiO$_{x}$ phase space, with colors representing varying oxygen concentrations. (b) 2D histograms of the PCA-decomposed TiO$_{x}$ phase space, with occurrence rate (colors) overlayed as a third dimension. Occurrence rate is defined as the likelihood of a structure from a given PCA grid occurring in the overall phase space. Dashed lines in (b) provide visual context for the approximate boundary of each phase, where a bin contains greater than 50 \% of a specific phase.}
    \label{fig:PCAspace}
\end{figure}

The ability to clearly distinguish between sub-spaces, in such a complex phase space, provides us with the ability to analyze these systems in more detail. For example, in Fig. \ref{fig:PCAspace}(b), we can observe which part of the phase space represents the equilibrium configurations encountered within each sub-space, as well as the outlier regions. This provides us with the ability to estimate the probability of each region contained in the phase space from occurring at a given temperature. Here, we can see that the TiO$_{2}$ and TiO$_{1.85}$ sub-spaces exist in slightly different topological spaces, with TiO$_{2}$ experiencing larger oscillations about its equilibrium point than TiO$_{1.85}$. We can also observe a clear trend in that, as the oxygen concentration is decreased, the oscillations about a given chemistry's equilibrium point are reduced, implying a smaller overall phase space. 

These oscillations provide insight into the size of a given oxygen concentration's portion of the overall phase space. For example, the TiO$_{1.85}$ phase space is visually more circular than the TiO$_{2}$ phase space, shown in Fig. \ref{fig:PCAspace}. with a smaller radius from the center of the approximated clustering shown in  \ref{fig:PCAspace} (b). This would seem to indicate that structures can deviate from the equilibrium configuration by a greater extent in TiO$_{2}$ than in TiO$_{1.85}$. These differences could play an important role in regard to H diffusion, as these oscillations about the equilibrium point may provide escape pathways, or trapping sites, that can ultimately make diffusion throughout the phase space more energetically favorable, or energetically unlikely.

\subsection{Effects of oxygen concentration}

The role of oxygen concentration was studied by observing the probability of 2F, 3F, and 4F O atoms within the system. All structures analyzed here are again taken from the 1,944-atom AFNN MD  trajectories. Fig. \ref{fig:PCACN} provides a picture of how the coordination number of various oxygen sites changes as a function stoichiometry. The axis presented in Fig. \ref{fig:PCACN} represents a 2-dimensional histogram of the PCA space. Within each histogram bin lives configurations of atoms present in the phase space. For each structure, the amount of 2F, 3F, and 4F present in the bin and are represented by the colors in Fig. \ref{fig:PCACN}. A Hermite interpolation scheme \cite{DEBOOR1987269} is used to smoothen the boundaries of each histogram bin to provide a more continuous color gradient.

From Fig. \ref{fig:PCACN} one can observe that the amount of 2F coordinated oxygen present in a system is highly correlated with the oxygen concentration with a negative linear relationship existing between the oxygen concentration and 2F oxygen probability. As seen in Fig. \ref{fig:PCACN} (a) 2F O sites exist more frequently throughout the structure at TiO$_{2}$ when compared to TiO$_{1.85}$. This decrease is quantified by observing the change in average probability along the x-axis, where $P($TiO$_{2}$$) =$ 30\% and $P($TiO$_{1.85}$$) =$ 23\%. The amount of 4F O atoms is also correlated with the oxygen concentration, with a linear trend existing between the two, as seen in Fig. \ref{fig:PCACN} (c). Here, for the case of 4F O atoms, $P($TiO$_{2}$$) =$ 9\% and $P($TiO$_{1.85}$$) =$ 12\%. Based on the results shown in Fig. \ref{fig:PCACN} (b) there is no apparent correlation between the oxygen concentration and the amount of 3F O present within the system.

\begin{figure}
       \centering
    	\includegraphics[trim={0 9cm 0 0cm},width=1.0\textwidth]{Figures/OCN.pdf}
    	\caption{2D histograms of the PCA-decomposed TiO$_{x}$ phase space, with coordination number probabilities (colors) overlayed as a third dimension. Coordination number probabilities represent the likelihood of an atom having the specified coordination number within a structure that is contained within a given PCA grid. (a), (b), and (c) represent 2F, 3F, and 4F oxygen CN environments respectively.}
    \label{fig:PCACN}
\end{figure}

The concentrations of the various O sites can also be used to verify the NMR results obtained by experiments. As stated previously, quantification analysis of the experimental peak areas reveals fractions of 14.78\%, 39.15\%, and 14.68\%. for 2F, 3F, and 4F O respectively. These fractions, when combined with the probabilities in Fig. \ref{fig:PCACN}, indicate that the experimental sample could be slightly oxygen reduced. We emphasize here that the analysis shown in Fig. \ref{fig:PCACN} can be used in conjunction with experiments to aid in the validation of the characterization of the sample.

We also note that the spatial connectivity of coordination networks (ex: the connected network of 2F oxygen atoms within some volume) appears to be stoichiometry dependant, a point which will be discussed in more detail in the following sections. This implies that one could tailor the connectivity of the potentially long-range coordination networks simply by reducing the oxygen content within the sample. However, we emphasize that while the trend in 2F and 4F ratios as a function of stoichiometry appears linear up to TiO$_{1.85}$, we do not explore samples with $x$ \textless 1.85, and therefore cannot make assertions regarding this regime.

\subsection{Hydrogen binding energies}

Using the 96 atom AFNN MD configurations a VGOP was calculated for each structure. Then for the first 2 PCA components of the VGOP features, K-means clustering was performed using 25 initial centroid placements. Once optimized, each point in the PCA space, which again represents an entire amorphous configuration, was binned into the corresponding K-means cluster. Stochastic random sampling was then used to down-select points from each cluster until the desired number of configurations was chosen. During the first pass, each K-means bin had the same number of points sampled from them. In the event that a cluster did not have the requested number of points, all points were taken. During the second pass the remaining number of requested points were evenly divided into each remaining cluster. This process was repeated until the total number of points requested had been chosen.

We computed H binding energies for the down-selected a-TiO$_{2}$ and a-TiO$_{1.88}$ structures (approximately 15,000 configurations), described in the previous section, to understand how hydrogen is incorporated in amorphous titania. Here, a neutral H atom (H$^{0}$) was used to examine its binding interaction in oxide, where the incorporated H$^{0}$ becomes one proton (H$^{+}$) absorbed on the O site and one electron reducing a nearby Ti; note that we did not assess the formation of hydride (H$^{-}$) on the Ti, since hydrogen thermodynamically prefers to exist as a proton (H$^{+}$) on the O site compared to a hydride (H$^{-}$) on the Ti site \cite{doi:10.1021/acs.jpcc.8b05251}. Fig.  \ref{fig:Hbind} provides plotted data for the case of a-TiO$_{2}$, while a-TiO$_{1.88}$ information can be found in the supplemental information.

Here we examine how the local oxygen coordination (O-Ti local networks) affects the hydrogen binding environment. Fig.  \ref{fig:Hbind}(a) shows the relaxed hydrogen bonding geometries (H-O-Ti$_{n}$, $n$=[2,4]) for the 2F, 3F, and 4F coordinated O site, respectively.  For the 2F coordinated O, we found that H preferentially binds to the apex of Ti-O-Ti bond normal to the Ti-O-Ti plane, whereas, for the 3F coordinated O, H-O-Ti$_{3}$ forms a sp$^{3}$-like pyramidal configuration; on the other hand, H bonding on the 4F coordinated O is highly distorted and not well characterized.  The difference in preferential H bonding direction can be attributed to differences in the hybridization of oxygen for the different coordination environment and resulting spatial distribution of the lone pair electrons of O \cite{MUSCENTI200570}. Previous DFT studies have demonstrated that there are two lone pairs (which are continuously distributed near the apex  of Ti-O-Ti bond) for the 2F oxygen and only one lone pair for 3F, by visualizing their electron localization function. This is also consistent with earlier theoretical study reporting that hydrogen (proton) bonding to O for oxygen-containing molecules tends to lie in the directions of the lone pair orbitals \cite{doi:10.1021/ja00316a034}. 

\begin{figure}
       \centering
    	\includegraphics[trim={0 0cm 0 0cm},width=1.0\textwidth]{Figures/HT_binding_energies.pdf}
    	\caption{(a) Histograms of the hydrogen binding energies for the various CN environments. Values shown here are the absolute number of samples, signifying the significant reduction in data set size for 4F environments. Values are color coded based on the CN environment. The dashed vertical lines indicate the mean for the distributions. (b) Fitted hydrogen binding energies for TiO$_{2}$. The fits were obtained using a powernorm distribution as part of the SciPy package \cite{2020SciPy-NMeth}. The distributions are colored according to the coordination number of the particular oxygen site. Here, the x-axis represents the binding energy, while the y-axis represents the probability of that binding energy occurring with respect to the number of environments for that CN type. The dashed black line represents the hydrogen binding energy in crystalline rutile. Inserted images in (a) show the oxygen environments encountered by hydrogen in the amorphous TiO$_{2}$ phase space.}
    \label{fig:Hbind}
\end{figure} 

Fig.  \ref{fig:Hbind}(b) demonstrates the distribution of H binding energies (E$_{b}$) for each O CN in a-TiO$_{2}$. The E$_{b}$ is calculated as follows: E$_{b} = $ E(a-TiO$_{x} /$ H) – E(a-TiO$_{x}$) – $\frac{1}{2}$ E(H$_{2}$), where E(a-TiO$_{x}/$H) and E(a-TiO$_{x}$) represent total energies of a-TiO$_{x}$ ($x$ = 2 or 1.88) with and without the H binding, respectively, while E(H$_{2}$) is the energy of a hydrogen gas molecule. This definition implies that a binding energy's strength will increase the value trends further away from zero, in the negative direction. 

As shown in Fig.  \ref{fig:Hbind}(b), the E$_{b}$ is strongly dependent on the O CN and H preferentially binds to lower coordinated O sites; the lower the E$_{b}$ gives the stronger H binding. Given that two lone pairs for the 2F O and one lone pair for the 3F O, stronger H binding for the 2F O could be partly attributed to a higher lone pair electron density. The fitted distributions provide us with expected values for each CN site. For the case of TiO$_{2}$ we see E$_{b}$ of (2F) -0.47 eV, (3F) 0.03 eV, and (4F) 0.51 eV. For the case of TiO$_{1.88}$ we obtain E$_{b}$ of (2F) -0.36 eV, (3F) 0.04 eV, and (4F) 0.49 eV. These values indicate that there is little-to-no difference in the binding energy when moving to a system with a lower oxygen concentration. This implies that the electronic structure of the local oxygen environment remains similar when reducing the oxygen content in the system. It is possible that this trend continues to system with even lower oxygen concentrations, though a thorough investigation of such systems is not performed in this work.

Our computed E$_{b}$ values include both proton binding on the oxygen site that is strongly dependent on the oxygen CN and electron localization energy on the Ti site that is largely determined by the lowest unoccupied electron state in the system (a-TiO$_{x}$). Thus, the variation of E$_{b}$ is mostly associated with the proton binding energy on the O site, while the electron localization energy is nearly identical within the same model structure.

Finally, the E$_{b}$ in rutile is calculated to be 0.29 eV for comparison, which suggests that the H binding in rutile is much weaker than the majority of H binding in a-TiO$_{2}$.  Although O in rutile is 3F coordinated similar to that in a-TiO$_{2}$, the weaker H binding in rutile could be explained by the higher strain energy cost to form a sp$^{3}$-like pyramidal configuration as well as the smaller electron localization energy in rutile compared to that in a-TiO$_{2}$. Note that for a single excess electron, the computed energy difference between the small polaron and delocalized electron configuration is around 0.1 eV for rutile, which agrees well with previous calculation \cite{https://doi.org/10.1002/pssr.201206464}. However, this value is much smaller than the energy gain by forming a small polaron configuration in a-TiO$_{2}$ for an excess electron, which can be as large as 0.8 eV from our calculations. W also provide binding energy values for single H within 216 atom unit cells in the supplementary information, to examine the effects of hydrogen concentration on the binding energy.

Here, we speculate the existence of two scenarios in which the hydrogen diffusivity could be affected by the hydrogen binding energy. First, if hydrogen is bonded to a particular oxygen atom, which is in turn surrounded by oxygen sites with higher CN, then there is an increased likelihood that H must hop into a more energetically unfavorable environment due to the shift towards weaker hydrogen binding. In this scenario, we speculate that slow diffusion could occur. However, if the opposite scenario exists, in which the H is surrounded by oxygen sites with lower CN, then the likelihood of moving into a more energetically favorable environment exists, potentially leading to fast diffusion. Second, H hopping within a similar CN environment (ex: 2F to 2F hopping), could lead to extremely fast diffusion if oxygen sites exist at similar points along the binding energy spectrum. Therefore, we speculate the existence of diffusion "highways", where fast diffusion occurs along similar CN networks. However, we also speculate the existence of transition networks, where H hops between different CN environments that have similar binding energies. 

We also speculate that stoichiometry may play a role in H diffusion, as the concentration of different CN environments could impact the connectivity of longer-range networks. For example, if 2F-2F networks drive H diffusion in TiO$_{2}$, they may exhibit different behavior due to the reduced number of 2F O sites in reduced oxygen samples. Based on this, there may be a correlation between the oxygen concentration of the sample and H diffusivity. We note, however, that a detailed understanding of H hopping kinetics and long-range diffusion is left for future work.



%It is perhaps important to summarize that we speculate the existence of two scenarios in which the hydrogen diffusivity becomes rate limited. The first being the presence of an abundance of 2F sites, which is found in the case of TiO$_{2}$. In this scenario, the existence of many sites exhibiting strong binding leads to an abundance of trapping sites, where hydrogen must overcome a large potential energy barrier in order to break the OH bond. The second scenario exists when the oxygen concentration is reduced and the amount of 2F is reduced while the presence of 4F is increased. In this scenario, due to the introduction of many energetically unfavorable binding sites (4F) hydrogen must again overcome a large potential energy barrier, though here it is required to form the OH bond. Both OH bond breaking and bond formation can lead to hydrogen trapping, depending on the rate of such sites around a hydrogen atom's current location. As the amount of such sites present in the amorphous system is dependant on the oxygen concentration, one can argue that trapping due to OH bond breaking is more likely to occur at high oxygen concentrations, while trapping due to OH bond formation is more likely to occur as the oxygen concentration is reduced.

    

%\begin{figure}
%       \centering
%    	\includegraphics[trim={4cm 0cm 4cm 0cm},width=.85\textwidth]{Figures/NMR.pdf}
%    	\caption{}
%    \label{fig:AFNN}
%\end{figure}


%As the DFT predicted hydrogen binding energies indicate stronger binding to two-fold coordinated oxygen atoms, in both the stoichiometric and non-stoichiometric cases, one can reason that systems that contain more 2F coordinated oxygen atoms should yield slower hydrogen diffusion. This is due to the average residence time of a hydrogen at a given oxygen site being intuitively longer for a site with stronger binding energy. Stronger binding energy also indicates that a larger potential energy barrier must be overcome for the O-H bond to break, prior to the hydrogen atom hopping between oxygen sites. The role of kinetics is not studied in this work. however, as we aim to examine how thermodynamic energies and structural differences could affect diffusion, independent of potential kinetic factors.

%This implies that as the oxygen concentration is decreased, the average binding energy contained within the system should trend towards weaker overall binding. Kinetically, this could translate to an increase in the number of energetically unfavorable sites, prohibiting certain pathways at low temperatures and increasing the average residence time. Qualitatively, this would indicate that hydrogen diffusion should be faster in the stoichiometric cases due to the potential reduction in average hydrogen residence time at a given oxygen site, due to the increased concentration of thermodynamically favorable sites.

 %The increase in the amount of 4F sites as the oxygen concentration is reduced could also lead to an increase in the average hydrogen residence time at a given oxygen site. As 4F sites show much weaker hydrogen binding, regardless of the stoichiometry, any increase in their concentration will populate the system with energetically unfavorable sites, again making kinetic pathways higher in energy. This could ultimately lead to slower hydrogen diffusion throughout the non-stoichiometric system. The correlation in the concentrations of 2F and 4F coordinated oxygen atoms also makes intuitive sense from a geometric perspective, as the removal of oxygen atoms creates free-volume in the system. This free-volume ultimately results in the dispersion of chemical species within the system and a small shift in the Ti-O peak of the radial distribution function, indicating the presence of more titanium atoms within a given oxygen atom's coordination sphere. The comparison between structural differences of stoichiometric and non-stoichiometric configurations can be found in the supplemental information.

  
